PipeOrgan: Efficient Inter-operation Pipelining with Flexible Spatial Organization and Interconnects

Because of the recent trends in Deep Neural Networks (DNN) models being memory-bound, inter-operator pipelining for DNN accelerators is emerging as a promising optimization. Inter-operator pipelining reduces costly on-chip global memory and off-chip memory accesses by forwarding the output of a layer as the input of the next layer within the compute array, which is proven to be an effective optimization by previous works. However, the design space of inter-operator pipelining is huge, and the space is not yet fully explored. In particular, identifying the right depth and granularity of pipelining (or no pipelining at all) is significantly dependent on the layer shapes and data volumes of weights and activations, and these are different even within a domain. Moreover, works divide the substrate into large chunks and map one layer onto each chunk, which requires communicating halfway through or through the global buffer. However, for fine-grained inter-operation pipelining, placing the corresponding consumer of the next layer tile close to the producer tile of the current layer is a better way to exploit fine-grained spatial reuse. In order to support variable number of layers (ie the right depth) and support multiple spatial organizations of layers (in accordance with the pipelining granularity) on the substrate, we propose PipeOrgan, a new class of spatial data organization strategy for energy efficient and congestion-free communication between the PEs for various pipeline depth and granularity. PipeOrgan takes advantage of flexible spatial organization and can allocate layers to PEs based on the granularity of pipelining. We also propose changes to the conventional mesh topology to improve the performance of coarse-grained allocation. PipeOrgan achieves 1.95x performance improvement over the state-of-the-art pipelined dataflow on XR-bench workloads.

==> 03-b-This_work.tex <==
\section{Framework for Variable Pipelining}

%\RG{A para expanding the figure}

In this work, we focus on choosing the optimal depth and optimal granularity of pipelining for running Deep Learning models on a spatial accelerator. Our framework takes in a DAG of operations as an input as~\autoref{fig:Toolflow} shows. Using~\DataflowNamee, we first determine the optimal depth of pipelining for different regions of the model and the intra-operation dataflows depending on the layer shapes which also influences the pipeline granularity. Based on the output of ~\DataflowNamee, ~\DataflowName determines the spatial allocation of layers onto the PEs, which consequently determines the configuration of the flexible NoC. 

We also study various traffic patterns for variable spatial allocations based on depths and granularities, for different DNN models ranging from image classification to language models. We show common traffic patterns as a result of variable depth and granularity and we propose a flexible NoC that optimizes the inter and intra operation communication with minumum area overhead.

\insertWideFigure{Toolflow}{Flow of the proposed dataflow and architecture for variable depth and granularity pipelining.}



==> Not-here-Arch.tex <==
\section{Accelerator}
\label{sec:arch}

\subsection{Overview}

The Conjugate Gradient accelerator consists of multliple nodes connected via the inter-node interconnect as shown in \TODO{}.

\subsubsection{System Configuration of a Node}

An accelerator node has the configuration close to the AMD Epyc CPU that is used in NVIDIA Selene. The configuration for a single node is shown in ~\autoref{tables:config}.
\input{tables/config.tex}


%\subsection{Matrix Operation Dataflows}

==> tables/config_backup.tex <==
\begin{scriptsize}
    \begin{table}[h!]
\begin{scriptsize}
    
  \begin{center}
  \caption{Configurations for workloads and architecture} 
  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{table:config}
  \begin{centering}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Parameter} & \textbf{Value}  \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Bytes per word/element & 1B (8 bits)\\\hline
    PE array size & 32$\times$32\\ 
    \hline
    PE dot product size\footnote{No reduction for grouped convolutions} & 8\\\hline
  %  PE array size at scale (\autoref{fig:scale}) & 256$\times$256\\ \hline
  % PE dot product size at scale (\autoref{fig:scale}) & 32\\\hline
    SRAM capacity & 1MB \\\hline
 %  SRAM capacity at scale (\autoref{fig:scale}) & 8MB\\ \hline
%    Off-chip bandwidth & \\\hline
 %   On-chip bandwidth & \\\hline
  %  Inter-cluster bandwidth & \\\hline
   Memory bandwidth & 256 GB/s\\\hline
 %   Memory bandwidth at scale (\autoref{fig:scale}) & 1TB/s\\\hline
    %Total L2 capacity & 32MB\\ \hline
    %Total L3 capacity & 256MB\\ \hline
  \end{tabular}
\vspace{-3mm}
\end{centering}
\end{center}
\end{scriptsize}

\end{table}
\end{scriptsize}

==> tables/related_work.tex <==
\begin{table}[ht!]
\begin{scriptsize}
\begin{center}
\caption{Related work table showing prior works related to mapping exploration and multi-layer acceleration.}
\label{tables:related}

{%\tt
\begin{tabular}{|c|c|c|}\hline
 \textbf{Prior Work} & \textbf{Pipeline} & \textbf{Main Contributions}  \\\hline
 Planaria~\cite{planaria} &  \redcheck  & Multi-tenant accelerator\\\hline
 AI-MT~\cite{AIMT}  & \redcheck  & Multi-tenant accelerator
 %\\ & reduction tree
% & & &
 \\\hline

 GAMMA~\cite{kao2020gamma} &  \redcheck & Mapper

 %\\ & unit
 %& & &
 \\\hline

MAESTRO~\cite{kwon2019understanding} & \redcheck  & Cost model\\\hline

 CoSA~\cite{cosa} &  \redcheck  &  Mapper\\\hline
 
 MAGMA~\cite{magma} &  \redcheck  & HDA Framework \\\hline
 Herald & \redcheck & HDA Framework\\\hline

 Atomic Dataflow~\cite{atomic-dataflow} &  \greencheck  & Intra-operation mapper\\\hline

 Stream~\cite{genetic-pipeline} & \greencheck & HDA Framework\\\hline

  HyGCN~\cite{yan2020hygcn}  & \greencheck  & Accelerator\\\hline

EnGN~\cite{liang2020engn}
 & \greencheck & Accelerator, fine-grained fusion.\\\hline   OMEGA~\cite{garg2021understanding} & \greencheck  &  Cost model\\\hline

   TANGRAM~\cite{tangram} &  \greencheck   & New Dataflow\\\hline

    FusedCNN~\cite{fusedcnn} & \greencheck  & Accelerator\\\hline


SET~\cite{isca-pip} &  \greencheck  & Mapper\\\hline

TileFlow~\cite{tileflow} &\greencheck & Mapper \\\hline


    \DataflowName (This work) &  \greencheck &  NoC and Spatial Organization \\\hline




\end{tabular}
}
\end{center}
\end{scriptsize}
\vspace{-0.1cm}
%'Sp' prefix implies support for zero skipping. IP=Inner Product, OP=Outer Product, Gust=Gustavsons}
\vspace{-0.15cm}
\end{table}
